Volumetric and Multi-View CNNs for Object Classification on 3D Data

3D shape models are becoming widely available and easier to capture, making available 3D information crucial for progress in object classification. Current state-of-the-art methods rely on CNNs to address this problem. Recently, we witness two types of CNNs being developed: CNNs based upon volumetric representations versus CNNs based upon multi-view representations. Empirical results from these two types of CNNs exhibit a large gap, indicating that existing volumetric CNN architectures and approaches are unable to fully exploit the power of 3D representations. In this paper, we aim to improve both volumetric CNNs and multi-view CNNs according to extensive analysis of existing approaches. To this end, we introduce two distinct network architectures of volumetric CNNs. In addition, we examine multi-view CNNs, where we introduce multi-resolution filtering in 3D. Overall, we are able to outperform current state-of-the-art methods for both volumetric CNNs and multi-view CNNs. We provide extensive experiments designed to evaluate underlying design choices, thus providing a better understanding of the space of methods available for object classification on 3D data.

==> cvpr16_3dcnn_arxiv (copy)/tex/abstract.tex <==

%We present a novel method utilizing convolutional neural networks on 3D data representations.
%We present a novel method -- it's really new, we promise!

3D shape models are becoming widely available and easier to capture, making available 3D information crucial for progress in object classification.
Current state-of-the-art methods rely on CNNs to address this problem. 
Recently, we witness two types of CNNs being developed: CNNs based upon volumetric representations versus CNNs based upon multi-view representations. 
Empirical results from these two types of CNNs exhibit a large gap, indicating that existing \DCNN architectures and approaches are unable to fully exploit the power of 3D representations. 
In this paper, we aim to improve both \DCNNs and \MVCNNs according to extensive analysis of existing approaches. 
To this end, we introduce two distinct network architectures of \DCNNs.
In addition, we examine \MVCNNs, where we introduce multi-resolution filtering in 3D.
Overall, we are able to outperform current state-of-the-art methods for both \DCNNs and \MVCNNs. 
We provide extensive experiments designed to evaluate underlying design choices, thus providing a better understanding of the space of methods available for object classification on 3D data.

\begin{comment}
The first network regularizes the learning process through the auxiliary learning task of predicting object labels from partial data; i.e., local regions of the 3D volumetric representation.
The second network introduces anisotropic probing kernels to capture long-range interactions between points on 3D shapes.
In our experiments, we demonstrate on both complete meshes and incomplete scans of real objects that our new architectures are able to significantly outperform existing 3D architectures.
\end{comment}

==> cvpr16_3dcnn_arxiv (copy)/tex/acknowledgement.tex <==
\mypara{Acknowledgement.} The authors gratefully acknowledge the support of Stanford Graduate Fellowship, NSF grants IIS-1528025 and DMS-1546206, ONR MURI grant N00014-13-1-0341, a Google Focused Research award, the Max Planck Center for Visual Computing and Communications and hardware donations by NVIDIA.

==> cvpr16_3dcnn_arxiv (copy)/tex/architecture.tex <==
\label{sec:DCNN}
\subsection{Overview}

We improve \DCNNs through three separate means: 1) introducing new network structures; 2) data augmentation; 3) feature pooling.

\paragraph{Network Architecture} 

We propose two network variations that significantly improve state-of-the-art CNNs on 3D volumetric data. 
% That is, in order to prevent overfitting, they are designed to enhance long-distance interactions in the early layers and suppress them in the late layers.
The first network is designed to mitigate overfitting by introducing auxiliary training tasks, which are themselves challenging. These auxiliary tasks encourage the network to predict object class labels from partial subvolumes. Therefore, no additional annotation efforts are needed.  %This strategy pushes the neural network to mine the data even if overfitting already happens for predicting the whole object. 
The second network is designed to mimic \MVCNNs, as they are strong in 3D shape classification. Instead of using rendering routines from computer graphics, our network projects a 3D shape to 2D by convolving its 3D volume with an anisotropic probing kernel. This kernel is capable of encoding long-range interactions between points. An image CNN is then appended to classify the 2D projection. Note that the training of the projection module and the image classification module is end-to-end. This emulation of \MVCNNs achieves similar performance to them, using only standard layers in CNN. 

In order to mitigate overfitting from too many parameters, we adopt the mlpconv layer from \cite{lin2013network} as our basic building block in both network variations.

%This helps capture the global structure of the 3D shape.
%Instead of using classical isotropic square kernels, we use an elongated kernel for the convolution operation in early stages and later change to normal square kernels. 
%Classical square kernels can only aggregate information from local isotropic vicinity, in 3D case, the occupancy is very sparse and it only contains limited discriminative information. 
%Our anisotropic kernel can encode such interactions at an early stage. 
%After the anisotropic convolutional layers, the 3D input is converted to be 2D, whose vicinity becomes denser with more discriminative information.
%Because we have cast the 3D problem to a 2D problem by CNN, we append an adapted network in network after the anisotropic filtering steps to address this 2D classification problem.
%\MATTHIAS{the latter part here seems wrong: I would like to avoid the phrasing casting 3D as 2D; it's not really what we doing, it's actually a much smarter way to extract the signal from a 3D volume with sparse information. We can probably also just skip it here as we need to shorten that part}

\paragraph{Data Augmentation} Compared with 2D image datasets, currently available 3D shape datasets are limited in scale and variation. To fully exploit the design of our networks, we augment the training data with different azimuth and elevation rotations. 
This allows the first network to cover local regions at different orientations, and the second network to relate distant points at different relative angles.
%As a comparison, the augmentation by 3DShapeNet \cite{shapenet2015v1} only introduces rotations along azimuth. 

\paragraph{Multi-Orientation Pooling} Both of our new networks are sensitive to shape orientation, i.e., they capture different information at different orientations. To capture a more holistic sense of a 3D object, we add an orientation pooling stage that aggregates information from different orientations. 


\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.8\linewidth]{./fig/probing.pdf}
	\caption{CNN with Anisotropic Probing kernels. We use an elongated kernel to convolve the 3D cube and aggregate information to a 2D plane. Then we use a 2D NIN (NIN-CIFAR10~\cite{lin2013network}) to classify the 2D projection of the original 3D shape. 
		\label{fig:anisotropic_probing}}
\end{figure*}

\subsection{Network 1: Auxiliary Training by Subvolume Supervision}
\label{sec:auxiliary_training}
We observe significant overfitting when we train the \DCNN proposed by \cite{wu20153d} in an end-to-end fashion (see supplementary). When the \DCNN overfits to the training data, it has no incentive to continue learning. We thus introduce auxiliary tasks that are closely correlated with the main task but are difficult to overfit, so that learning continues even if our main task is overfitted.  % Furthermore, if these auxiliary tasks are challenging, they will be hard to overfit and consume some capacity of the network, hence reduce the capacity for the main task to mitigate overfitting. Furthermore, 

%We design auxiliary training tasks following the above spirit. 
%Interestingly, each task we add still predicts the same object labels --- but it makes the prediction only based upon a local subvolume of the input.
These auxiliary training tasks also predict the same object labels, but the predictions are made solely on a local subvolume of the input.
Without complete knowledge of the object, the auxiliary tasks are more challenging, and can thus better exploit the discriminative power of local regions. This design is different from the classic multi-task learning setting of hetergenous auxiliary tasks, which inevitably requires collecting additional annotations (e.g., conducting both object classification and detection \cite{girshick2015fast}). 

We implement this design through an architecture shown in Fig~\ref{fig:auxiliary_training}. 
The first three layers are mlpconv (multilayer perceptron convolution) layers, a 3D extension of the 2D mlpconv proposed by \cite{lin2013network}. 
The input and output of our mlpconv layers are both 4D tensors. 
Compared with the standard combination of linear convolutional layers and max pooling layers, mlpconv has a three-layer structure and is thus a universal function approximator if enough neurons are provided in its intermediate layers. Therefore, mlpconv is a powerful filter for feature extraction of local patches, enhancing approximation of more abstract representations. In addition, mlpconv has been validated to be more discriminative with fewer parameters than ordinary convolution with pooling~\cite{lin2013network}. 

At the fourth layer, the network branches into two. 
The lower branch takes the whole object as input for traditional classification. 
The upper branch is a novel branch for auxiliary tasks. 
It slices the $512\times 2\times 2 \times 2$ 4D tensor ($2$ grids along $x$, $y$, $z$ axes and $512$ channels) into $2\times 2\times 2=8$ vectors of dimension $512$. We set up a classification task for each vector. 
A fully connected layer and a softmax layer are then appended independently to each vector to construct classification losses. Simple calculation shows that the receptive field of each task is $22\times 22\times 22$, covering roughly $2/3$ of the entire volume.

% Each of our auxiliary task must classify an object with only partial information, forcing the neural network to spend more efforts in scrutinizing the ``details'' of data, even if significant overfitting has already occured for the  prediction using the entire object.


\subsection{Network 2: Anisotropic Probing}
\label{sec:anisotropic_probing}
The success of \MVCNNs is intriguing. \MVCNNs first project 3D objects to 2D and then make use of well-developed 2D image CNNs for classification. Inspired by its success, we design a neural network architecture that is also composed of the two stages. However, while \MVCNNs use external rendering pipelines from computer graphics, we achieve the 3D-to-2D projection using network layers in a manner similar to `X-ray scanning'. 

Key to this network is the use of an elongated anisotropic kernel which helps capture the global structure of the 3D volume.
As illustrated in Fig~\ref{fig:anisotropic_probing}, the neural network has two modules: an anisotropic probing module and a network in network module. 
The anisotropic probing module contains three convolutional layers of elongated kernels, each followed by a nonlinear ReLU layer. 
Note that both the input and output of each layer are 3D tensors. 

In contrast to traditional isotropic kernels, an anisotropic probing module has the advantage of aggregating long-range interactions in the early feature learning stage with fewer parameters. % After this step, the resulting local vicinities become denser with more discriminative information, as opposed to local 3D vicinity, which is usually very sparse and lacks enough discriminative power. Similar to Network 1,  the modification of architecture in this network is also aiming at optimized discriminative power of local regions. 
As a comparison, with traditional neural networks constructed from isotropic kernels, introducing long-range interactions at an early stage can only be achieved through large kernels, which inevitably introduce many more parameters.
After anisotropic probing, we use an adapted NIN network \cite{lin2013network} to address the classification problem.
%This is similar to a projection to 2D; however, we show that anisotropic probing can efficiently learn this extraction step.\todo{check}

Our anistropic probing network is capable of capturing internal structures of objects through its X-ray like projection mechanism. This is an ability not offered by standard rendering. % that simulates visible lights. 
Combined with multi-orientation pooling (introduced below), it is possible for this probing mechanism to capture any 3D structure, due to its relationship with the Radon transform. 

In addition, this architecture is scalable to higher resolutions, since all its layers can be viewed as 2D. While 3D convolution involves computation at locations of cubic resolution, we maintain quadratic compute.

 \begin{figure}[b!]
 	\centering
 	\includegraphics[width=0.8\linewidth]{./fig/multi_orientation}
 	\caption{Left: Volumetric CNN (single orientation input). Right: Multi-orientation volumetric CNN (\MOVCNN), which takes in various orientations of the 3D input, extracts features from shared $\text{CNN}_1$ and then pass pooled feature through another network $\text{CNN}_2$ to make a prediction.}
 	\label{fig:multi_ori}
 \end{figure}
\subsection{Data Augmentation and Multi-Orientation Pooling} \label{sec:arch:aug}
The two networks proposed above are both sensitive to model orientation. In the subvolume supervision method, different model orientations define different local subvolumes; in the anisotropic probing method, only voxels of the same height and along the probing direction can have interaction in the early feature extraction stage. 
Thus it is helpful to augment the training data by varying object orientation and combining predictions through orientation pooling. 

Similar to \SuMVCNN~\cite{su15mvcnn} which aggregates information from multiple view inputs through a view-pooling layer and follow-on fully connected layers, we sample 3D input from different orientations and aggregate them in a multi-orientation volumetric CNN (\MOVCNN) as shown in Fig~\ref{fig:multi_ori}. At training time, we generate different rotations of the 3D model by changing both azimuth and elevation angles, sampled randomly. A volumetric CNN is firstly trained on single rotations. Then we decompose the network to $\text{CNN}_1$ (lower layers) and $\text{CNN}_2$ (higher layers) to construct a multi-orientation version. The \MOVCNN's weights are initialized by a previously trained volumetric CNN with $\text{CNN}_1$'s weights fixed during fine-tuning. While a common practice is to extract the highest level features (features before the last classification linear layer) of multiple orientations, average/max/concatenate them, and train a linear SVM on the combined feature, this is just a special case of the \MOVCNN.

Compared to~3DShapeNets~\cite{wu20153d} which only augments data by rotating around vertical axis, our experiment shows that orientation pooling combined with elevation rotation can greatly increase performance.




% \subsection{Virtual Scans and Incomplete Point Clouds}
% To deal with real scanning data, we do virtual scans of 3D meshes to get partial scanning data for training.

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{./fig/placeholder.pdf}
% \caption{Figure: showing training data and virtual scans. % \todo{First version due: Nov 3, 5PM PST. Angie, Mengyuan}}
% \label{fig:loss}
% \end{figure}



==> cvpr16_3dcnn_arxiv (copy)/tex/augmentation.tex <==
By adding elevation perturbation, combining features from multiple model rotations can greatly improve accuracy while training on data with only azimuth rotations combining helps little. 
\MATTHIAS{What exactly is elevation perturbation?}
It's interesting that add elevation perturbation actually does not improve performance for features extracted from one rotation, however the power of combined features is greatly boosted (without elevation, combining improves around $1\%$; with elevation, it's more than $3.5\%$).

==> cvpr16_3dcnn_arxiv (copy)/tex/conclusion.tex <==
In this paper, we have addressed the task of object classification on 3D data using \DCNNs and \MVCNNs.
We have analyzed the performance gap between \DCNNs and \MVCNNs from perspectives of network architecture and 3D resolution. 
The analysis motivates us to propose two new architectures of \DCNNs, which outperform state-of-the-art \DCNNs, achieving  comparable performance to \MVCNNs at the same 3D resolution of $30\times 30\times 30$.
Further evalution over the influence of 3D resolution indicates that 3D resolution is likely to be the bottleneck for the performance of \DCNNs. Therefore, it is worth exploring the design of efficient \DCNN architectures that scale up to higher resolutions. 



==> cvpr16_3dcnn_arxiv (copy)/tex/diagnosis.tex <==

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\linewidth,height=5cm]{./fig/placeholder.pdf}
%	\caption{Sphere rendering at different resolutions. }
%	\label{fig:data_representation}
%\end{figure}

 \begin{figure}[h]
 	\centering
 	\includegraphics[width=\linewidth]{./fig/vcnn_vs_mvcnn_existedwork.pdf}
 	\caption{Classification accuracy.  Yellow and blue bars:  Performance drop of \MVCNN due to discretization of CAD models in rendering. Blue and green bars: Volumetric CNN is significantly worse than \MVCNN, even though their inputs have similar amounts of information. This indicates that the network of the \DCNN is weaker than that of the \MVCNN.}
 	\label{fig:vcnn_vs_mvcnn}
 \end{figure}
 
Two representations of generic 3D shapes are popularly used for object classification, volumetric and multi-view (Fig~\ref{fig:data_representation}). The volumetric representation encodes a 3D shape as a 3D tensor of binary or real values. The multi-view representation encodes a 3D shape as a collection of renderings from multiple viewpoints. Stored as tensors, both representations can easily be used to train convolutional neural networks, i.e., \DCNNs and \MVCNNs. 

Intuitively, a volumetric representation should encode as much information, if not more, than its multi-view counterpart. However, experiments indicate that \MVCNNs produce superior performance in object classification. Fig~\ref{fig:vcnn_vs_mvcnn} reports the classification accuracy on the ModelNet40 dataset by state-of-the-art volumetric/multi-view architectures\footnote{We train models by replicating the architecture of \cite{wu20153d} for \DCNNs and \cite{su15mvcnn} for \MVCNNs. All networks are trained in an end-to-end fashion. All methods are trained/tested on the same split for fair comparison. The reported numbers are average instance accuracy. See Sec~\ref{sec:experiments} for details.}. A \DCNN based on voxel occupancy (green) is $7.3\%$ worse than a \MVCNN (yellow). 

We investigate this performance gap in order to ascertain how to improve \DCNNs. The gap seems to be caused by two factors: input resolution and network architecture differences. The \MVCNN down-samples each rendered view to $227\times 227$ pixels (Multi-view Standard Rendering in Fig~\ref{fig:data_representation}); to maintain a similar computational cost, the \DCNN uses a $30\times 30\times 30$ occupancy grid  (Volumetric Occupancy Grid in Fig~\ref{fig:data_representation})\footnote{Note that $30\times 30 \times 30 \approx 227 \times 227$.}. As shown in Fig~\ref{fig:data_representation}, the input to the \MVCNN captures more detail. 

However, the difference in input resolution is not the primary reason for this performance gap, as evidenced by further experiments.  We compare the two networks by providing them with data containing similar level of detail. To this end, we feed the \MVCNN with renderings of the $30\times 30\times 30$ occupancy grid using \emph{sphere rendering}\footnote{It is computationally prohibitive to match the \DCNN resolution to \MVCNN, which would be $227\times227\times 227$.}, i.e., for each occupied voxel, a ball is placed at its center, with radius equal to the edge length of a voxel (Multi-View Sphere Rendering in Fig~\ref{fig:data_representation}). We train the \MVCNN from scratch using these sphere renderings.
The accuracy of this \MVCNN is reported in blue.
 
\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.8\linewidth]{./fig/subvolume.pdf}
	\caption{Auxiliary Training by Subvolume Supervision (Sec~\ref{sec:auxiliary_training}). The main innovation is that we add auxiliary tasks to predict class labels that focus on part of an object, intended to drive the CNN to more heavily exploit local discriminative features. An mlpconv layer is a composition of three conv layers interleaved by ReLU layers. The five numbers under mlpconv are the number of channels, kernel size and stride of the first conv layer, and the number of channels of the second and third conv layers, respectively. The kernel size and stride of the second and third conv layers are $1$. For example, $\text{mlpconv}(48,6,2; 48; 48)$ is a composition of $\text{conv}(48, 6, 2)$, ReLU, $\text{conv}(48, 1, 1)$, ReLU, $\text{conv}(48, 1, 1)$ and ReLU layers.  Note that we add dropout layers with rate=$0.5$ after fully connected layers.}
	\label{fig:auxiliary_training}
\end{figure*}

As shown in Fig~\ref{fig:vcnn_vs_mvcnn}, even with similar level of object detail, the \DCNN (green) is $4.8\%$ worse than the \MVCNN (blue). That is, \emph{there is still significant room to improve the architecture of \DCNNs}. This discovery motivates our efforts in Sec~\ref{sec:DCNN} to improve \DCNNs. Additionally, low-frequency information in 3D seems to be quite discriminative for object classification---it is possible to achieve $89.5\%$ accuracy (blue) at a resolution of only $30\times 30\times 30$. This discovery motivates our efforts in Sec~\ref{sec:mvcnn} to improve \MVCNNs with a 3D multi-resolution approach.


==> cvpr16_3dcnn_arxiv (copy)/tex/experiment.tex <==

We evaluate our \DCNNs and \MVCNNs along with current state of the art on the ModelNet dataset~\cite{wu20153d} and a new dataset of real-world reconstructions of 3D objects.


For convenience in following discussions, we define \emph{3D resolution} to be the discretization resolution of a 3D shape. That is, a $30\times 30\times 30$ volume has 3D resolution $30$. The sphere rendering from this volume also has 3D resolution $30$, though it may have higher 2D image resolution.

\subsection{Datasets}
% Introduce both ModelNet40 and our real scanning data set. Mention ShapeNet as well.
\paragraph{ModelNet} 
We use ModelNet~\cite{wu20153d} for our training and testing datasets. ModelNet currently contains $127,915$ 3D CAD models from $662$ categories. ModelNet40, a subset including $12,311$ models from $40$ categories, is well annotated and can be downloaded from the web. The authors also provide a training and testing split on the website, in which there are $9,843$ training and $2,468$ test models\footnote{VoxNet~\cite{maturana2015voxnet} uses the train/test split provided on the website and report average class accuracy on the $2,468$ test split. 3DShapeNets~\cite{wu20153d} and MVCNN~\cite{su15mvcnn} use another train/test split comprising the first 80 shapes of each category in the ``train'' folder (or all shapes if there are fewer than 80) and the first 20 shapes of each category in the ``test'' folder, respectively.}. We  use this train/test split for our experiments. 

By default, we report classification accuracy on all models in the test set (average instance accuracy). For comparisons with previous work we also report average class accuracy.
 

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./fig/dataset.pdf}
	\caption{Example models from our real-world dataset. Each model is a dense 3D reconstruction, annotated, and segmented from the background.}
	\label{fig:dataset}
\end{figure}

\paragraph{Real-world Reconstructions} 
We provide a new real-world scanning dataset benchmark, comprising 243 objects of 12 categories; the geometry is captured with an ASUS Xtion Pro and a dense reconstruction is obtained using the publicly-available VoxelHashing framework \cite{niessner2013real}.
For each scan, we have performed a coarse, manual segmentation of the object of interest.
In addition, each scan is aligned with the world-up vector.
While there are existing datasets captured with commodity range sensors -- e.g., \cite{silberman2012indoor,xiao2013sun3d,song2015sun} -- this is the first containing hundreds of annotated models from dense 3D reconstructions.
The goal of this dataset is to provide an example of modern real-time 3D reconstructions; i.e., structured representations more complete than a single RGB-D frame but still with many occlusions. This dataset is used as a test set.


\subsection{Comparison with State-of-the-Art Methods}
\label{sec:exp:comparison_ingroup}
We compare our methods with state of the art for shape classification on the ModelNet40 dataset.
In the following, we discuss the results within \DCNN methods and within \MVCNN methods.
% A discussion of results across these methods can be found in Sec~\ref{sec:exp:comparison_acrossgroup}.
%Methods in comparison are grouped by input type -- volumetric representation and multi-view representation. In the following we discuss the results within each group. The discussion into results across groups can be found in Sec~\ref{sec:exp:comparison_acrossgroup}.   



\paragraph{Volumetric CNNs}
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./fig/volumetric_results}
	\caption{Classification accuracy on ModelNet40 (voxelized at resolution 30). Our \DCNNs have matched the performance of \MVCNN at 3D resolution $30$ (our implementation of \SuMVCNN~\cite{su15mvcnn}, rightmost group).}
	\label{fig:volumetric_results}
\end{figure}
Fig~\ref{fig:volumetric_results} summarizes the performance of \DCNNs. Ours-MO-SubvolumeSup is the subvolume supervision network in Sec~\ref{sec:auxiliary_training} and Ours-MO-AniProbing is the anistropic probing network in Sec~\ref{sec:anisotropic_probing}. Data augmentation is applied as described in Sec~\ref{sec:exp:augmentation} (azimuth and elevation rotations). For clarity, we use MO- to denote that both networks are trained with an additional multi-orientation pooling step ($20$ orientations in practice). For reference of \MVCNN performance at the same 3D resolution, we also include Ours-MVCNN-Sphere-30, the result of our \MVCNN with sphere rendering at 3D resolution $30$. More details of setup can be found in the supplementary. % For consistency of other experiments and previous works, we measure the performance by both average class accuracy and average instance accuracy. 

As can be seen, both of our proposed volumetric CNNs significantly outperform state-of-the-art volumetric CNNs. Moreover, they both match the performance of our \MVCNN under the same 3D resolution. That is, \emph{the gap between \DCNNs and \MVCNNs is closed} under 3D resolution $30$ on ModelNet40 dataset, an issue that motivates our study (Sec~\ref{sec:diagnosis}). 

\paragraph{Multi-view CNNs}
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./fig/mvcnn_results}
	\caption{Classification acurracy on ModelNet40 (multi-view representation). The 3D multi-resolution version is the strongest. It is worth noting that the simple baseline HoGPyramid-LFD performs quite well.}
	\label{fig:mvcnn_results}
\end{figure}
Fig~\ref{fig:mvcnn_results} summarizes the performance of \MVCNNs. Ours-MVCNN-MultiRes is the result by training an SVM over the concatenation of fc7 features from Ours-MVCNN-Sphere-30, 60, and Ours-MVCNN. HoGPyramid-LFD is the result by training an SVM over a concatenation of HoG features at three 2D resolutions. Here LFD (lightfield descriptor) simply refers to extracting features from renderings. Ours-MVCNN-MultiRes achieves state-of-the-art.



\subsection{Effect of 3D Resolution over Performance}
\label{sec:exp:comparison_acrossgroup}
Sec~\ref{sec:exp:comparison_ingroup} shows that our \DCNN and \MVCNN performs comparably at 3D resolution $30$. Here we study the effect of 3D resolution for both types of networks. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=\linewidth]{./fig/resolution_mvcnn}
	\caption{Top: sphere rendering at 3D resolution $10$, $30$, $60$, and standard rendering. Bottom: performance of image-based CNN and volumetric CNN with increasing 3D resolution. The two rightmost points are trained/tested from standard rendering.}
	\label{fig:resolution_mvcnn}
\end{figure}

Fig~\ref{fig:resolution_mvcnn} shows the performance of our \DCNN and \MVCNN at different 3D resolutions (defined at the beginning of Sec~\ref{sec:experiments}). Due to computational cost, we only test our \DCNN at 3D resolutions $10$ and $30$. The observations are: first,  the performance of our \DCNN and \MVCNN is on par at tested 3D resolutions; second, the performance of \MVCNN increases as the 3D resolution grows up. To further improve the performance of \DCNN, this experiment suggests that it is worth exploring how to scale \DCNN to higher 3D resolutions.

\subsection{More Evaluations}
\paragraph{Data Augmentation and Multi-Orientation Pooling}
\label{sec:exp:augmentation}
We use the same \DCNN model, the end-to-end learning verion of 3DShapeNets~\cite{wu20153d}, to train and test on three variations of augmented data (Table~\ref{tb:augmentation}). Similar trend is observed for other volumetric CNN variations.  

\begin{table}[h!]
	\small
	\centering
	\begin{tabular}{lccc}
		\hline
		Data Augmentation & Single-Ori & Multi-Ori & $\Delta$\\
		\hline
		Azimuth rotation (AZ) & $84.7$ & $86.1$ & $1.4$\\
		AZ + translation& $84.8$ & $86.1$ & $1.3$\\
		AZ + elevation rotation & $83.0$ & $\mathbf{87.8}$ & $4.8$\\
		\hline
	\end{tabular}
	\caption{Effects of data augmentations on multi-orientation volumetric CNN. We report numbers of classification accuracy on ModelNet40, with (Multi-Ori) or without (Single-Ori) multi-orientation pooling described in Sec~\ref{sec:arch:aug}.}
	\label{tb:augmentation}
\end{table}
When combined with multi-orientation pooling, applying both azimuth rotation (AZ) and elevation rotation (EL) augmentations is extremely effective. Using only azimuth augmentation (randomly sampled from $0^{\circ}$ to $360^{\circ}$) with orientation pooling, the classification performance is increased by $86.1\%-84.7\%=1.4\%$; combined with elevation augmentation (randomly sampled from $-45^{\circ}$ to $45^{\circ}$), the improvement becomes more significant -- increasing by $87.8\%-83.0\%=4.8\%$. On the other hand, translation jittering (randomly sampled shift from $0$ to $6$ voxels in each direction) provides only marginal influence.

% By default, we use azimuth and elevation augmented data and use multi-orientation volumetric CNN (\MOVCNN) to aggregate them. By default we use 20 orientations for \MOVCNN.

\paragraph{Comparison of Volumetric CNN Architectures}
The architectures in comparison include VoxNet~\cite{maturana2015voxnet},  E2E-\cite{wu20153d} (the end-to-end learning variation of \cite{wu20153d} implemented in Caffe~\cite{jia2014caffe} by ourselves), 3D-NIN (a 3D variation of Network in Network~\cite{lin2013network} designed by ourselves as in Fig~\ref{fig:auxiliary_training} without the ``Prediction by partial object'' branch), SubvolumeSup (Sec~\ref{sec:auxiliary_training}) and AniProbing (Sec~\ref{sec:anisotropic_probing}).  Data augmentation of AZ+EL (Sec~\ref{sec:exp:augmentation}) are applied. 

From Table~\ref{tb:perf},  first, the two \DCNNs we propose, SubvolumeSup and AniProbing networks, both show superior performance, indicating the effectiveness of our design;
second, multi-orientation pooling increases performance for all network variations. This is especially significant for the anisotropic probing network, since each orientation usually only carries partial information of the object. 

\begin{table}
	\small
	\centering
	\begin{tabular}{l|cc}
		\hline
		Network & Single-Ori & Multi-Ori \\
		\hline
		E2E-\cite{wu20153d} & $83.0$ & $87.8$ \\
		VoxNet\cite{maturana2015voxnet} & $83.8$ & $85.9$ \\
		\hline
		3D-NIN & $86.1$ & $88.5$ \\
		Ours-SubvolumeSup & $\mathbf{87.2}$ & $89.2$  \\
		Ours-AniProbing & $85.9$ & $\mathbf{89.9}$  \\
		\hline
	\end{tabular}
	\caption{Comparison of performance of volumetric CNN architectures. Numbers reported are classification accuracy on ModelNet40. Results from E2E-\cite{wu20153d} (end-to-end learning version) and VoxNet~\cite{maturana2015voxnet} are obtained by ourselves. All experiments are using the same set of azimuth and elevation augmented data.}
	\label{tb:perf}
\end{table}

\paragraph{Comparison of Multi-view Methods}


\begin{table}[b!]
	\small
	\centering
	\begin{tabular}{l|ccc}
		\hline
		Method & \#Views & \begin{tabular}[c]{@{}l@{}}Accuracy\\(class)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Accuracy\\(instance)\end{tabular}\\
		\hline
		SPH~(reported by \cite{wu20153d}) & - & $68.2$ & - \\
		LFD~(reported by \cite{wu20153d}) & - & $75.5$ & - \\
		FV (reported by \cite{su15mvcnn}) & 12 & $84.8$ & - \\
		\SuMVCNN~\cite{su15mvcnn} & 80 & $90.1$ & - \\
		\hline
		PyramidHoG-LFD & 20 & $87.2$ & $90.5$\\
		Ours-MVCNN & 20 & $89.7$ & $92.0$\\
	    Ours-MVCNN-MultiRes & 20 & $\mathbf{91.4}$ & $\mathbf{93.8}$ \\
		\hline
	\end{tabular}
	\caption{Comparison of multi-view based methods. Numbers reported are classification accuracy (class average and instance average) on ModelNet40.}
	\label{tb:multiview_performance}
\end{table}

We compare different methods that are based on multi-view representations in Table~\ref{tb:multiview_performance}. Methods in the second group are trained on the full ModelNet40 train set. Methods in the first group, SPH, LFD, FV, and \SuMVCNN, are trained on a subset of ModelNet40 containing 3,183 training samples. They are provided for reference. Also note that the \AbbrMVCNNs in the second group are our implementations in Caffe with AlexNet instead of VGG as in \SuMVCNN~\cite{su15mvcnn}. 

We observe that \AbbrMVCNNs are superior to methods by SVMs on hand-crafted features. 
%
%We perform various experiments to analyze the \MVCNN representation and its strengths.
%We analyze our \MVCNN (c.f. Sec~\ref{sec:mvcnn}) along with several existing multi-view approaches: multi-view HOG, the SPH and LFD representations of \cite{wu20153d}, and the \MVCNN approach of \cite{su15mvcnn}. 
%
%We first investigate the effect of pre-training with the ImageNet external RGB image dataset. To this end, we compare the performance of a multi-view CNN initialized with random parameters and one pre-trained on ImageNet (both trained on ModelNet40). 
%Table~\ref{tb:pretraining} shows that the randomly initialized \MVCNN maintains strong performance, indicating that the effect of ImageNet pre-training is marginal classification accuracy on ModelNet40, and that the \DCNN does need external knowledge to improve its performance.
%
%Additionally, we analyze the influence of the resolution of the 3D input data, to determine whether there is any loss in discretizing to the commonly used $30\times 30\times 30$ voxelization \cite{wu20153d, maturana2015voxnet}.
%To address this concern, we test a multi-view CNN under sphere rendering and multi-resolution 3D filtering, as described in Sec~\ref{sec:mvcnn}.
%Our \MVCNN with multi-resolution 3D filtering performs very strongly on both CAD models and real-world reconstructions (see Table~\ref{tb:pretraining}), showing that the $30\times 30\times 30$ voxelization preserves considerable discriminative power. 
%The discovery consolidates the choice of 3DShapeNet, VoxNet and our 3DCNN to use $30\times 30\times 30$ as the input. 


\paragraph{Evaluation on the Real-World Reconstruction Dataset}

\begin{table}[t!]
	\small
\begin{center}
    \begin{tabular}{l|c|c}
    \hline
    Method      & Classification & Retrieval MAP \\ \hline
    E2E-\cite{wu20153d} & $69.6$ & -\\
    \SuMVCNN~\cite{su15mvcnn} & $72.4$ & $35.8$\\
    \hline
    Ours-MO-SubvolumeSup & $73.3$ & $39.3$\\
    Ours-MO-AniProbing & $70.8$ & $40.2$\\
    Ours-MVCNN-MultiRes & $\mathbf{74.5}$ & $\mathbf{51.4}$\\
    \hline
    \end{tabular}
    \caption{Classification accuracy and retrieval MAP on reconstructed meshes of 12-class real-world scans.}
    \label{tb:real_eval}
\end{center}
\end{table}

We further assess the performance of \DCNNs and \MVCNNs on real-world reconstructions in Table~\ref{tb:real_eval}. All methods are trained on CAD models in ModelNet40 but tested on real data, which may be highly partial, noisy, or oversmoothed~(Fig~\ref{fig:dataset}).
Our networks continue to outperform state-of-the-art results. In particular, our 3D multi-resolution filtering is quite effective on real-world data, possibly because the low 3D resolution component filters out spurious and noisy micro-structures. Example results for object retrieval can be found in supplementary.

%\subsection{Feature Visualization}
%\begin{figure}[h]
%\centering
%\includegraphics[width=\linewidth]{./fig/placeholder.pdf}
%\caption{Figure: kernel visualization - What is a good way to visualize?}
%\label{fig:kernel_vis}
%\end{figure}


==> cvpr16_3dcnn_arxiv (copy)/tex/introduction.tex <==


%motivate why 3D is important
%Object classification from 2D monocular images has been one of the most researched problems in computer vision.
%It is particularly relevant as it is fundamental to many vision systems, spanning a wide field of application scenarios from self-driving cars to autonomous robots.
%While traditional approaches, such as deformable part models \cite{felzenszwalb2010cascade}, rely on hand-crafted feature descriptors, significant progress has been made using deep learning \cite{russakovsky2014imagenet}.
%Given enough training data, feature learning has shown to be more effective than feature engineering \todo{cite?}.


Understanding 3D environments is a vital element of modern computer vision research due to paramount relevance in many vision systems, spanning a wide field of application scenarios from self-driving cars to autonomous robots.
Recent advancements in real-time SLAM techniques and crowd-sourcing of virtual 3D models have additionally facilitated the availability of 3D data. \cite{silberman2012indoor,xiao2013sun3d,song2015sun,wu20153d,chang2015shapenet}.
This development has encouraged the lifting of 2D to 3D for deep learning, opening up new opportunities with the additional information of 3D data; e.g., aligning models is easier in 3D Euclidean space. 
In this paper, we specifically focus on the object classification task on 3D data obtained from both CAD models and commodity RGB-D sensors.
In addition, we demonstrate retrieval results in the supplemental material.

%Additionally, a CNN architecture allows local geometric regularity to be characterized by local kernels.
%Such architectures are also easily generalizable to myriad types of data, including occupancy grids, distance fields, and signed distance fields, as well as easily applicable to different recognition tasks through interchanging different loss functions.

%3D is challenging -- existing methods don't do it well
While the extension of 2D convolutional neural networks to 3D seems natural, the additional
computational complexity (volumetric domain) and data sparsity introduces significant challenges; for instance, in an image, every pixel contains observed information, whereas in 3D, a shape is only defined on its surface.
Seminal work by Wu et al. \cite{wu20153d} propose \DCNN architectures on volumetric grids for object classification and retrieval.
While these approaches achieve good results, it turns out that training a CNN on multiple 2D views achieves a significantly higher performance, as shown by Su et al. \cite{su15mvcnn}, who augment their 2D CNN with pre-training from ImageNet RGB data \cite{deng2009imagenet}.
These results indicate that existing 3D CNN architectures and approaches are unable to fully exploit the power of 3D representations.
In this work, we analyze these observations and evaluate the design choices.
Moreover, we show how to reduce the gap between \DCNNs and \MVCNNs by efficiently augmenting training data, introducing new CNN architectures in 3D.
Finally, we examine \MVCNNs; our experiments show that we are able to improve upon state of the art with improved training data augmentation and a new multi-resolution component.
%which fundamentally work in 3D.
%, and generalize to all common 3D volumetric representations \todo{check: occupancy, SDF, DF}.

\paragraph{Problem Statement}
We consider volumetric representations of 3D point clouds or meshes as input to the 3D object classification problem. 
This is primarily inspired by recent advances in real-time scanning technology, which use volumetric data representations.
%\ANGIE{maybe also mention that volumetric encompasses a variety of representations/generaliable? don't know if necessary} 
%\MATTHIAS{we need to mention that we operate on binary grids that can be derived from signed and unsigned distanced fields.}
%Typically, the representation is obtained through discretization to occupancy grids (\rqi{may include normals as well, if time permits}), (truncated) distance fields or (truncated) signed distance field.  
We further assume that the input data is already pre-segmented by 3D bounding boxes. 
In practice, these bounding boxes can be extracted using the sliding windows, object proposals, or background subtraction. 
The output of the method is the category label of the volumetric data instance.

\paragraph{Approach}
We provide a detailed analysis over factors that influence the performance of \DCNNs, including network architecture and volumn resolution. Based upon our analysis, we strive to improve the performance of \DCNNs. 
We propose two \DCNN network architectures that signficantly improve state-of-the-art of volumetric CNNs on 3D shape classification. \emph{This result has also closed the gap between \DCNNs and \MVCNNs}, when they are provided with 3D input discretized at $30\times 30\times 30$ 3D resolution. 
The first network introduces auxiliary learning tasks by classifying part of an object, which help to scrutize details of 3D objects more deeply.
The second network uses long anisotropic kernels to probe for long-distance interactions. Combining data augmentation with a multi-orientation pooling, we observe significant performance improvement for both networks.
We also conduct extensive experiments to study the influence of volume resolution, which sheds light on future directions of improving \DCNNs. 

Furthermore, we introduce a new multi-resolution component to \MVCNNs, which improves their already compelling performance.

In addition to providing extensive experiments on 3D CAD model datasets, we also introduce a dataset of real-world 3D data, constructed using dense 3D reconstruction taken with \cite{niessner2013real}. Experiments show that our networks can better adapt from synthetic data to this real-world data than previous methods.

%To sum up, our contributions are
%\begin{itemize}
%	\item \vspace{-0.2cm}a detailed analysis of the network architectures of \DCNNs,
%	\item \vspace{-0.2cm}two new network architectures of \DCNNs that achieve state-of-the-art peformance among \DCNNs ,
%	\item \vspace{-0.2cm}improved performance on \MVCNNs using multi-resolution filtering in 3D,
%	\item \vspace{-0.2cm}a new test dataset comprising 3D data of over 240 real-world objects.\vspace{-0.2cm}
%\end{itemize}


% % % % %

% % % % % 
%\begin{figure}[h]
%\centering
%\includegraphics[width=\linewidth]{./fig/representation.png}
%\caption{3D shape representations used in this paper. }
%\label{fig:data_representation}
%\end{figure}




==> cvpr16_3dcnn_arxiv (copy)/tex/mvcnn.tex <==
The \MVCNN proposed by \cite{su15mvcnn} is a strong alternative to volumetric representations. 
This multi-view representation is constructed in three steps: first, a 3D shape is rendered into multiple images using varying camera extrinsics; then image features (e.g. $\text{conv5}$ feature in VGG or AlexNet) are extracted for each view; lastly features are combined across views through a pooling layer, followed by fully connected layers. 
% This facilitates capturing long-range 3D interactions by analyzing a 2D local neighborhood, as distant connections are made through the 3D-to-2D projection.
% In fact, our anisotropic probing approach (c.f. Sec~\ref{sec:anisotropic_probing}) achieves a similar effect, which allows our approach to bridge the performance gap between \DCNN and \MVCNN.

% Another advantage of \MVCNNs is that the conversion to 2D allows exploitation of existing approaches for feature learning from 2D images; for instance, \cite{su15mvcnn} pre-train their model using features from ImageNet \cite{deng2009imagenet}.

Although the \MVCNN presented by \cite{su15mvcnn} produces compelling results, we are able to improve its performance through a multi-resolution extension with improved data augmentation.
We introduce multi-resolution 3D filtering to capture information at multiple scales. We perform \emph{sphere rendering} (see Sec~\ref{sec:diagnosis}) at different volume resolutions. Note that we use spheres for this discretization as they are view-invariant. % To achieve multi-resolution filtering, we perform this sphere rendering at multiple resolutions of discretized spheres, thus capturing a variety of signals across the resolutions.
In particular, this helps regularize out potential noise or irregularities in real-world scanned data (relative to synthetic training data), enabling robust performance on real-world scans. Note that our 3D multi-resolution filtering is different from classical 2D multi-resolution approaches, since the 3D filtering respects the distance in 3D. 

Additionally, we also augment training data with variations in both azimuth and elevation, as opposed to azimuth only. We use AlexNet instead of VGG for efficiency.
% This allows a greater variety of distant interactions to be captured.
% In contrast, \cite{su15mvcnn} changes tilt with less azimuth and elevation variation, and instead uses max pooling.

% Finally, we use average pooling of the last layer and retrain an SVM, whereas \cite{su15mvcnn} uses max pooling together with a second CNN.

% Overall, these improvements allow us to improve performance over existing state-of-the-art \cite{su15mvcnn}.
%In particular, on real-world test data, our results are more than \todo{XY} accurate (cf. Fig. \todo{XY}).




==> cvpr16_3dcnn_arxiv (copy)/tex/problem.tex <==


\MATTHIAS{move to intro and shorten; and adapt it accordingly to our new story}

% 3D feature learning on point cloud data. start from object classification. 
Since the classification problem is fundamental to most vision systems, we focus our study of 3D neural network architecture on tackling this problem. 

The input data format is a volumetric representation of 3D point clouds or meshes.
Typically, the representation is obtained through discretization to occupancy grids (\rqi{may include normals as well, if time permits}), (truncated) distance fields or (truncated) signed distance field.  
We further assume that the input data is already pre-segmented by 3D bounding boxes. 
In practice, these bounding boxes can be extracted using the sliding shape method \todo{CITE JIANXIONG}, object proposals or background subtraction (e.g., in Google driverless cars). 

The output of the system is the category label of the volumetric data instance.

While this problem has been approached through the use of classic features and learning models, we choose to solve this problem using convolutional neural networks (CNNs).
%; CNNs are a good choice for our problem, compared with classic features and learning models. 
That is \ANGIE{wording}, given enough training data, feature learning has shown to be more effective than feature engineering.
Recent advancements in crowd-sourcing and 3d sensor technology has enabled us to acquire  colloections of increasing numbers of 3D meshes and point clouds, such as those of ShapeNet and ModelNet \ANGIE{cite?}.
Additionally, a CNN architecture allows local geometric regularity to be characterized by local kernels.
Such architectures are also easily generalizable to myriad types of data, including occupancy grids, distance fields, and signed distance fields, as well as easily applicable to different recognition tasks through interchanging different loss functions.




==> cvpr16_3dcnn_arxiv (copy)/tex/relatedwork.tex <==

\paragraph{Shape Descriptors}
A large variety of shape descriptors has been developed in the computer vision and graphics community.
For instance, shapes can be represented as histograms or bag-of-feature models which are constructed from surface normals and curvatures \cite{horn1984extended}.
Alternatives include models based on distances, angles, triangle areas, or tetrahedra volumes \cite{osada2002shape}, local shape diameters measured at densely-sampled surface points \cite{chaudhuri2010data}, Heat kernel signatures \cite{bronstein2011shape,kokkinos2012intrinsic}, or extensions of SIFT and SURF feature descriptors to 3D voxel grids \cite{knopp2010hough}.
The spherical harmonic descriptor (SPH) \cite{kazhdan2003rotation} and the Light Field descriptor (LFD) \cite{chen2003visual} are other popular descriptors.
LFD extracts geometric and Fourier descriptors from object silhouettes rendered from several different viewpoints, and can be directly applied to the shape classification task.
In contrast to recently developed feature learning techniques, these features are hand-crafted and do not generalize well across different domains.


\begin{figure}[t!]
	\centering
	\includegraphics[width=\linewidth]{./fig/representation.pdf}
	\caption{3D shape representations. }
	\label{fig:data_representation}
\end{figure}
\paragraph{Convolutional Neural Networks}

Convolutional Neural Networks (CNNs) \cite{lecun1998gradient} have been successfully used in different areas of computer vision and beyond.
In particular, significant progress has been made in the context of learning features.
It turns out that training from large RGB image datasets  (e.g., ImageNet \cite{deng2009imagenet}) is able to learn general purpose image descriptors that outperform hand-crafted features for a number of vision tasks, including object detection, scene recognition, texture recognition and classification \cite{donahue2013decaf,girshick2014rich,razavian2014cnn,cimpoi2014describing,han2015matchnet}.
This significant improvement in performance on these tasks has decidedly moved the field forward.

% CNNs have been also used to combine information form multiple RGB images; for instance recognizing 3D objects using two concatenated views (binocular images) as input \cite{lecun2004learning}, or to efficiently learn stereo matches for 3D reconstruction \cite{vzbontar2015stereo}.


\paragraph{CNNs on Depth and 3D Data}

%2.5
With the introduction of commodity range sensors, the depth channel became available to provide additional information that could be incorporated into common CNN architectures.
A very first approach combines convolutional and recursive neural networks for learning features and classifying RGB-D images \cite{socher2012convolutional}.
Impressive performance for object detection from RGB-D images has been achieved using a geocentric embedding for depth images that encodes height above ground and angle with gravity for each pixel in addition to the horizontal disparity \cite{gupta2014learning}.
Recently, a CNN architecture has been proposed where the RGB and depth data are processed in two separate streams; in the end, the two streams are combined with a late fusion network \cite{eitel15iros}.
All these descriptors operate on single RGB-D images, thus processing 2.5D data.


%actual 3D 
Wu et al. \cite{wu20153d} lift 2.5D to 3D with their 3DShapeNets approach by  categorizing each voxel as free space, surface or occluded, depending on whether it is in front of, on, or behind the visible surface (i.e., the depth 
value) from the depth map.
The resulting representation is a 3D binary voxel grid, which is the input to a CNN with 3D filter banks.
Their method is particularly relevant in the context of this work, as they are the first to apply CNNs on a 3D representation.
A similar approach is VoxNet \cite{maturana2015voxnet}, which also uses  binary voxel grids and a corresponding 3D CNN architecture.
% C(32, 5, 2)−C(32, 3, 1)−P(2)−F C(128)−F C(K); data augmentation for rotation with voting
The advantage of these approaches is that it can process different sources of 3D data, including LiDAR point clouds, RGB-D point clouds, and CAD models; we likewise follow this direction.



%backprojecting to 2D
An alternative direction is to exploit established 2D CNN architectures; to this end, 2D data is extracted from the 3D representation.
In this context, DeepPano \cite{shi2015deeppano} converts 3D shapes into panoramic views;  i.e., a cylinder projection around its principle axis.
Current state-of-the-art uses multiple rendered views, and trains a CNN that can process all views jointly \cite{su15mvcnn}.
This multi-view CNN (MVCNN) is pre-trained on ImageNet \cite{deng2009imagenet} and uses view-point pooling to combine all streams obtained from each view.
A similar idea on stereo views has been proposed earlier \cite{lecun2004learning}.
%In contrast to this 2D view-based approach, we aim to capture a 3D description of geometry; that is, describing both the surface geometry and the inner structure. \todo{check plz}
%\todo{disadvantage? rendering? performs poorly on real data?}

\begin{comment}
%
Sliding Shapes \cite{song2014sliding}
%shape databses
\\
\MATTHIAS{Shape Databases:}
NYU2 \cite{silberman2012indoor}
SUN-3D \cite{xiao2013sun3d}
SUN RGB-D \cite{song2015sun}

%dunno if we need this stuff: it's part-based assemply
\MATTHIAS{if we need this stuff: it's part-based assemply:}
Analyzing 3D CAD model collection using assembly-based approach to build deformable part-based models \cite{funkhouser2004modeling}, \cite{chaudhuri2011probabilistic}, \cite{kalogerakis2012probabilistic}.
These methods are limited to a specific class of shapes with small variations, with surface correspondence being one of the key problems in such approaches. 
\end{comment}



==> tex/augmentation.tex <==
By adding elevation perturbation, combining features from multiple model rotations can greatly improve accuracy while training on data with only azimuth rotations combining helps little. 
\MATTHIAS{What exactly is elevation perturbation?}
It's interesting that add elevation perturbation actually does not improve performance for features extracted from one rotation, however the power of combined features is greatly boosted (without elevation, combining improves around $1\%$; with elevation, it's more than $3.5\%$).

==> tex/problem.tex <==


\MATTHIAS{move to intro and shorten; and adapt it accordingly to our new story}

% 3D feature learning on point cloud data. start from object classification. 
Since the classification problem is fundamental to most vision systems, we focus our study of 3D neural network architecture on tackling this problem. 

The input data format is a volumetric representation of 3D point clouds or meshes.
Typically, the representation is obtained through discretization to occupancy grids (\rqi{may include normals as well, if time permits}), (truncated) distance fields or (truncated) signed distance field.  
We further assume that the input data is already pre-segmented by 3D bounding boxes. 
In practice, these bounding boxes can be extracted using the sliding shape method \todo{CITE JIANXIONG}, object proposals or background subtraction (e.g., in Google driverless cars). 

The output of the system is the category label of the volumetric data instance.

While this problem has been approached through the use of classic features and learning models, we choose to solve this problem using convolutional neural networks (CNNs).
%; CNNs are a good choice for our problem, compared with classic features and learning models. 
That is \ANGIE{wording}, given enough training data, feature learning has shown to be more effective than feature engineering.
Recent advancements in crowd-sourcing and 3d sensor technology has enabled us to acquire  colloections of increasing numbers of 3D meshes and point clouds, such as those of ShapeNet and ModelNet \ANGIE{cite?}.
Additionally, a CNN architecture allows local geometric regularity to be characterized by local kernels.
Such architectures are also easily generalizable to myriad types of data, including occupancy grids, distance fields, and signed distance fields, as well as easily applicable to different recognition tasks through interchanging different loss functions.



